SEAL : Interactive Tool for Systematic Error Analysis and Labeling

With the advent of Transformers, large language models (LLMs) have saturated well-known NLP benchmarks and leaderboards with high aggregate performance. However, many times these models systematically fail on tail data or rare groups not obvious in aggregate evaluation. Identifying such problematic data groups is even more challenging when there are no explicit labels (e.g., ethnicity, gender, etc.) and further compounded for NLP datasets due to the lack of visual features to characterize failure modes (e.g., Asian males, animals indoors, waterbirds on land, etc.). This paper introduces an interactive Systematic Error Analysis and Labeling (\seal) tool that uses a two-step approach to first identify high error slices of data and then, in the second step, introduce methods to give human-understandable semantics to those underperforming slices. We explore a variety of methods for coming up with coherent semantics for the error groups using language models for semantic labeling and a text-to-image model for generating visual features. SEAL toolkit and demo screencast is available at https://huggingface.co/spaces/nazneen/seal.

==> Theory/Theory_full.tex <==

\section{Theoretical analysis}
\label{sec:theory}
% In this section, we provide a stability analysis of the proposed SEAL. 
\paragraph{Overview} 
In this section, we provide theoretical guarantees for the stability of the proposed SEAL. More specifically, our stability theorem states that a small perturbation of the input of our Cluster+Summary error analysis pipeline (say using a slightly different test set for evaluation) would only cause a small difference of the clustering results [Step 2: Clustering], and a small difference in the error summary [Step 3:semantic labeling \& Step 4: Visual Feature Generation]. 

\lingjiao{Consider reorganizing the paper. It is a bit strange to have problem setup in the theoretical analysis section. It is supposed to be earlier in the paper.}
\paragraph{Problem Setup and Notations}
We ask: how does a small change in the input of the clustering $\{(x_i,y_i)\}_{i=1}^{n}$ affect the explanation tuple $M \triangleq \{m_k\}_{k=1}^{K}$. 
Here, $K$ denotes the number of explanations,$m_k\triangleq(w_k,s_k,a_k)$ encodes the $k$th explanation message, 
where $w_k, s_k$, and $a_k$ represent the sentence vector, the number of data points explained by this message, and the average accuracy among those data points. 
To answer this question, we first need a distance metric to measure how close two explanation messages are. 
\begin{definition}
Given any two explanation tuple $M=\{m_k\}_{k=1}^{K}$ and $M'=\{m_k'\}_{k=1}^{K}$, define a distance between them as 
\begin{equation*}
d_{\max}(M,M')\triangleq \max_{1\leq i\leq K} \min_{1 \leq j \leq K} d(m_i,m_i',m_j,m'_j)    
\end{equation*}
where 
\begin{equation*}
d(m_i,m'_i,m_j,m'_j)\triangleq \|m_i-m'_j\|_2 + \|m'_i-m_j\|_2    
\end{equation*}   
\end{definition}
Here, a small  distance value $d_{\max}$ implies a small difference in the explanation word vector, the size of each cluster, and the accuracy within each cluster. 
Now we are ready to present the stability result as follows.

\begin{theorem}
Let $S$ and $T$ denote two set of $n$ data points i.i.d. from some data distribution $P$. Suppose the probability space of $P$ is  compact with size $B$, and the density function of $P$ is lower-bounded away from 0 and upper bounded by some constant. 
Let $M_S$ and $M_T$ be the error messages generated by \seal{} with input $S$ and $T$. 
If $S$ and $T$ differs in $o(\sqrt{n})$ data points, and the the clustering algorithm always gives the exactly optimal solution, then we have 
\begin{equation*}
d_{\max}(M_S, M_T) \xrightarrow[]{P} 0     
\end{equation*}
\end{theorem}
Intuitively, this means that \seal{} is \textit{stable}: if the input data points are close enough, then the generated error messages are roughly the same. In other words, \seal{} is robust to small dataset noise.
This is particularly useful in an interactive environment, where users may frequently update a few points in the dataset and anticipate no major error message shifts in a time.


\begin{proof}
TODO. The proof sketch is very similar to the proof developed in lemma 5.1 in stable kmeans paper, except that now we need to consider both cluster centers and the size and error of each point. 
This should be done by ensuring, if two cluster centers are close enough, then only a small number of data points' classes may have been changed. The details need a bit more work though.
\end{proof}


%%%%%%%%%%%%%%

\noindent \textbf{Proposition 5.1}
Assume the density of $P$ (with respect to the Lebesgue measure $\lambda$ over $\mathcal{Z}$ ) is bounded away from 0, i.e. $d P>c d \lambda$ for some $c>0$. Suppose the clusterings $A$ and $B$ are minimizers of the $K$-means objective $W(C)$ over the sets $S$ and $T$, respectively. Suppose that $|S \triangle T|=o(\sqrt{n})$. Then
$$
d_{\max }\left(\left\{a_{1}, \ldots, a_{K}\right\},\left\{b_{1}, \ldots, b_{K}\right\}\right) \stackrel{P}{\longrightarrow} 0 .
$$
Hence, the centers of the minimizers of the within-point scatter are stable with respect to perturbations of $o(\sqrt{n})$ points. 




%%%%%%%%%%%%%%



 


%%%%%%%%%%%%%%%

